Stochastic Order Redshift Technique (SORT): a simple, efficient and robust method to improve cosmological redshift measurements

We present a simple, efficient and robust approach to improve cosmological redshift measurements. The method is based on the presence of a reference sample for which a precise redshift number distribution (dN/dz) can be obtained for different pencil-beam-like sub-volumes within the original survey. For each sub-volume we then impose: (i) that the redshift number distribution of the uncertain redshift measurements matches the reference dN/dz corrected by their selection functions; and (ii) the rank order in redshift of the original ensemble of uncertain measurements is preserved. The latter step is motivated by the fact that random variables drawn from Gaussian probability density functions (PDFs) of different means and arbitrarily large standard deviations satisfy stochastic ordering. We then repeat this simple algorithm for multiple arbitrary pencil-beam-like overlapping sub-volumes; in this manner, each uncertain measurement has multiple (non-independent) "recovered" redshifts which can be used to estimate a new redshift PDF. We refer to this method as the Stochastic Order Redshift Technique (SORT). We have used a state-of-the-art N-body simulation to test the performance of SORT under simple assumptions and found that it can improve the quality of cosmological redshifts in an efficient and robust manner. Particularly, SORT redshifts are able to recover the distinctive features of the 'cosmic web' and can provide unbiased measurement of the two-point correlation function on scales > 4 Mpc/h. Given its simplicity, we envision that a method like SORT can be incorporated into more sophisticated algorithms aimed to exploit the full potential of large extragalactic photometric surveys.

==> figs/hist_comparisons.tex <==
 
    \begin{figure}
    
    \begin{minipage}{0.45\textwidth}
    \centering
    \includegraphics[width=\textwidth]{../figs/{hist_comp_fg0.3_angsep1_dz0.0003}.pdf}
    \end{minipage}
    \caption{Normalized distribution (arbitrary binning of $0.0005$) 
    of the redshift differences with
respect to the true redshift $z_{\rm true}$, for both the observed
($z_{\rm obs}$; black lines) and the recovered $z_{\rm new}$  (red
lines) redshifts, using a reference sample of $f_{\rm ref} = 5\%$. The
left and right panels present the normalized counts in a linear and
logarithmic scale, respectively. Our proposed method considerably
reduce the redshift uncertainty for a considerable fraction of the
data, and it is virtually never worse than the original estimation.}
\label{fig:hist_comparison}
\end{figure}

==> figs/information_pie.tex <==
 \begin{figure*}
    \begin{minipage}{0.32\textwidth}
    \centering
    \includegraphics[width=1.01\textwidth]{../figs/{pie_diagram_fg0.3_angsep1_dz0.0003_zctrl}.pdf}
    \end{minipage}
        \begin{minipage}{0.32\textwidth}
    \centering
    \includegraphics[width=1.01\textwidth]{../figs/{pie_diagram_fg0.3_angsep1_dz0.0003_zsort}.pdf}
    \end{minipage}
    \begin{minipage}{0.32\textwidth}
    \centering
    \includegraphics[width=1.01\textwidth]{../figs/{pie_diagram_fg0.3_angsep1_dz0.0003_zsortp}.pdf}
    \end{minipage}
    
    \caption{Pie diagrams for our different methods: [...XXX]}.

\label{fig:information_pie}

\end{figure*}


==> figs/shape.tex <==
 \begin{figure*}
    
    \begin{minipage}{0.48\textwidth}
    \centering
    \includegraphics[width=1.01\textwidth]{../figs/{hist_zbins_zph_fg0.3_angsep1_dz0.0003}.pdf}
    \end{minipage}
    \begin{minipage}{0.48\textwidth}
    \centering
    \includegraphics[width=1.01\textwidth]{../figs/{hist_zbins_zsort_fg0.3_angsep1_dz0.0003}.pdf}
    \end{minipage}
    
    \caption{Redshift difference $\Delta z \equiv z-z_{\rm true}$
using different redshift bins within our survey: [...XXX] . The left
panel shows the results using $z = z_{\rm ph}$ (original photometric
sample), while the right panel shows the results using $z = z_{\rm
sort}$ (\sort)}..

\label{fig:shape}

\end{figure*}
